High-Dimensional Bayesian Optimization via Semi-Supervised Learning with Optimized Unlabeled Data Sampling

We introduce a novel semi-supervised learning approach, named Teacher-Student Bayesian Optimization ($\texttt{TSBO}$), integrating the teacher-student paradigm into BO to minimize expensive labeled data queries for the first time. $\texttt{TSBO}$ incorporates a teacher model, an unlabeled data sampler, and a student model. The student is trained on unlabeled data locations generated by the sampler, with pseudo labels predicted by the teacher. The interplay between these three components implements a unique selective regularization to the teacher in the form of student feedback. This scheme enables the teacher to predict high-quality pseudo labels, enhancing the generalization of the GP surrogate model in the search space. To fully exploit $\texttt{TSBO}$, we propose two optimized unlabeled data samplers to construct effective student feedback that well aligns with the objective of Bayesian optimization. Furthermore, we quantify and leverage the uncertainty of the teacher-student model for the provision of reliable feedback to the teacher in the presence of risky pseudo-label predictions. $\texttt{TSBO}$ demonstrates significantly improved sample-efficiency in several global optimization tasks under tight labeled data budgets.

==> subfile_tab7.tex <==
\begin{table}[tbp]
    \centering
    \caption{The ablation test of \ourmethod\ on the Chemical Design Task with 250 new queries}
    
    \begin{tabular}{l c c c c c}
    \toprule
    Method   &  PL predictor & Student & $\zsetunlabel$ Sampling &  Penalized LogP ($\uparrow$ )\\
    \midrule
    T-LBO \citep{grosnit2021tlbo}  & - & -  & -  & 5.695±1.25 \\
    \midrule
    \multirow{2}{*}{TSBO w/o student's feedback}
      % & \makecell{MLP}   & - & \makecell{Uniform}  & -\\
      & \makecell{MLP}   & - & \makecell{Gaussian}  & 9.917±6.251\\
      % & \makecell{Prob-MLP}  & - & \makecell{Gaussian}  & 17.557±6.998\\
     &  Oracle    & - & \makecell{Gaussian}  & 26 @ 100 queries\\
    \midrule
    \multirow{5}{*}{TSBO}
      & \makecell{Prob-MLP}  & \makecell{UA-GP} & \makecell{Uniform}  &4.881±1.416\\
      & \makecell{MLP} & GP & \makecell{Optimized  Gaussian}  & 12.568±7.965\\    
      & \makecell{Prob-MLP} & \makecell{GP}  & \makecell{Optimized  Gaussian}  & 21.115±6.382 \\
      & \makecell{Prob-MLP}  & \makecell{UA-GP} & \makecell{Gaussian} &23.464±9.535\\

      & \makecell{Prob-MLP} & \makecell{UA-GP}  & \makecell{Optimized  Gaussian} & 25.020±4.794 \\
    \bottomrule
    \end{tabular}
    %}
    \label{tab:full-ablation}
\end{table}

